Optimal Beam Training for mmWave Massive MIMO using 802.11ay

Beam training of 802.11 ad is a technology that helps accelerate the analog weighting vector (AWV) selection process under the constraint of the existing code-book for AWV. However, 5G milli-meter wave (mmWave) multiple-input-multiple-output (MIMO) system brings challenges to this new technology due to the higher order of complexity of antennae. Hence, the existing codebook of 11ad is unlikely to even include the near-optimal AWV and the data rate will degrade severely. To cope with this situation, this paper proposed a new beam training protocol combined with the state-of-the-art compressed sensing channel estimation in order to find the AWV to maximize the optimal data-rate. Simulation is implemented to show the data-rate of AWV achieved by 11 ad is worse than the proposed protocol.

==> ref.tex <==
@article{pi2011introduction,
  title={An introduction to millimeter-wave mobile broadband systems},
  author={Pi, Zhouyue and Khan, Farooq},
  journal={IEEE communications magazine},
  volume={49},
  number={6},
  pages={101--107},
  year={2011},
  publisher={IEEE}
}

@article{xiao2016hierarchical,
  title={Hierarchical codebook design for beamforming training in millimeter-wave communication},
  author={Xiao, Zhenyu and He, Tong and Xia, Pengfei and Xia, Xiang-Gen},
  journal={IEEE Transactions on Wireless Communications},
  volume={15},
  number={5},
  pages={3380--3392},
  year={2016},
  publisher={IEEE}
}
@article{ghasempour2017ieee,
  title={IEEE 802.11 ay: Next-generation 60 GHz communication for 100 Gb/s Wi-Fi},
  author={Ghasempour, Yasaman and da Silva, Claudio RCM and Cordeiro, Carlos and Knightly, Edward W},
  journal={IEEE Communications Magazine},
  volume={55},
  number={12},
  pages={186--192},
  year={2017},
  publisher={IEEE}
}



@article{gao2016energy,
  title={Energy-efficient hybrid analog and digital precoding for mmWave MIMO systems with large antenna arrays},
  author={Gao, Xinyu and Dai, Linglong and Han, Shuangfeng and Chih-Lin, I and Heath, Robert W},
  journal={IEEE Journal on Selected Areas in Communications},
  volume={34},
  number={4},
  pages={998--1009},
  year={2016},
  publisher={IEEE}
}

@article{goldsmith2003capacity,
  title={Capacity limits of MIMO channels},
  author={Goldsmith, Andrea and Jafar, Syed Ali and Jindal, Nihar and Vishwanath, Sriram},
  journal={IEEE Journal on selected areas in Communications},
  volume={21},
  number={5},
  pages={684--702},
  year={2003},
  publisher={IEEE}
}

@inproceedings{alkhateeb2013hybrid,
  title={Hybrid precoding for millimeter wave cellular systems with partial channel knowledge},
  author={Alkhateeb, Ahmed and El Ayach, Omar and Leus, Geert and Heath, Robert W},
  booktitle={2013 Information Theory and Applications Workshop (ITA)},
  pages={1--5},
  year={2013},
  organization={IEEE}
}

@article{el2017,
  title={“Spatially sparse precoding in millimeter wave MIMO systems,” IEEE Journ},
  author={El Ayach, Omar and Rajagopal, Sridhar and Abu-Surra, Shadi},
  journal={Selected Areas of Comm},
  volume={8},
  number={3},
  year={2017}
}


@article{molisch2017hybrid,
  title={Hybrid beamforming for massive MIMO: A survey},
  author={Molisch, Andreas F and Ratnam, Vishnu V and Han, Shengqian and Li, Zheda and Nguyen, Sinh Le Hong and Li, Linsheng and Haneda, Katsuyuki},
  journal={IEEE Communications Magazine},
  volume={55},
  number={9},
  pages={134--141},
  year={2017},
  publisher={IEEE}
}


@inproceedings{perahia2010ieee,
  title={IEEE 802.11 ad: Defining the next generation multi-Gbps Wi-Fi},
  author={Perahia, Eldad and Cordeiro, Carlos and Park, Minyoung and Yang, L Lily},
  booktitle={2010 7th IEEE consumer communications and networking conference},
  pages={1--5},
  year={2010},
  organization={IEEE}
}


@article{xiao2013suboptimal,
  title={Suboptimal spatial diversity scheme for 60 GHz millimeter-wave WLAN},
  author={Xiao, Zhenyu},
  journal={IEEE Communications Letters},
  volume={17},
  number={9},
  pages={1790--1793},
  year={2013},
  publisher={IEEE}
}

@inproceedings{xia2008practical,
  title={Practical antenna training for millimeter wave MIMO communication},
  author={Xia, Pengfei and Niu, Huaning and Oh, Jisung and Ngo, Chiu},
  booktitle={2008 IEEE 68th Vehicular Technology Conference},
  pages={1--5},
  year={2008},
  organization={IEEE}
}

@inproceedings{xia2008multi,
  title={Multi-stage iterative antenna training for millimeter wave communications},
  author={Xia, Pengfei and Yong, Su-Khiong and Oh, Jisung and Ngo, Chiu},
  booktitle={IEEE GLOBECOM 2008-2008 IEEE Global Telecommunications Conference},
  pages={1--6},
  year={2008},
  organization={IEEE}
}


@inproceedings{khan2011mmwave,
  title={mmWave mobile broadband (MMB): Unleashing the 3--300GHz spectrum},
  author={Khan, Farooq and Pi, Zhouyue},
  booktitle={34th IEEE Sarnoff Symposium},
  pages={1--6},
  year={2011},
  organization={IEEE}
}


@article{zhang2022architecture,
  title={Architecture-Algorithmic Trade-offs in Multi-path Channel Estimation for mmWAVE Systems},
  author={Zhang, Lyutianyang and Roy, Sumit and Cao, Liu},
  journal={arXiv preprint arXiv:2209.02944},
  year={2022}
}
